Large Language Models-Aided Program Debloating

As software grows in complexity to accommodate diverse features and platforms, software bloating has emerged as a significant challenge, adversely affecting performance and security. However, existing approaches inadequately address the dual objectives of debloating: maintaining functionality by preserving essential features and enhancing security by reducing security issues. Specifically, current software debloating techniques often rely on input-based analysis, using user inputs as proxies for the specifications of desired features. However, these approaches frequently overfit provided inputs, leading to functionality loss and potential security vulnerabilities. To address these limitations, we propose LEADER, a program debloating framework enhanced by Large Language Models (LLMs), which leverages their semantic understanding, generative capabilities, and decision-making strengths. LEADER mainly consists of two modules: (1) a documentation-guided test augmentation module designed to preserve functionality, which leverages LLMs to comprehend program documentation and generates sufficient tests to cover the desired features comprehensively, and (2) a multi-advisor-aided program debloating module that employs a neuro-symbolic pipeline to ensure that the security of the software can be perceived during debloating. This module combines debloating and security advisors for analysis and employs an LLM as a decision-maker to eliminate undesired code securely. Extensive evaluations on widely used benchmarks demonstrate the efficacy of LEADER. These results demonstrate that LEADER surpasses the state-of-the-art tool CovA in functionality and security. These results underscore the potential of LEADER to set a new standard in program debloating by effectively balancing functionality and security.

==> algorithm/UnusedCodeElimination.tex <==
% \begin{algorithm}
% \caption{Unused Code Elimination}
% \KwIn{CFG $cfg$ containing all code blocks}
% \KwOut{Optimized CFG with dead code removed}

% \SetKwFunction{InitWorklist}{initialize\_worklist}
% \SetKwFunction{AnalyzeBlock}{analyze\_block}
% \SetKwFunction{IsDeadCode}{is\_dead\_code}
% \SetKwFunction{RemoveStmt}{remove\_statement}

% \SetKwProg{Fn}{Function}{:}{end}
% \SetKwComment{Comment}{$\triangleright$\ }{}

% \BlankLine
% $DUChain \leftarrow BuildDefUseChain(P)$\;
% \InitWorklist{$worklist$, $cfg$}\;
% \While{$worklist$ is not empty}{
%     $block \leftarrow worklist$.pop()\;
%     $du\_chain \leftarrow$ \AnalyzeBlock{$block$}\;
%     \ForEach{statement $stmt$ in $block$}{
%         \If{\IsDeadCode{$stmt$, $du\_chain$}}{
%             \RemoveStmt{$block$, $stmt$}\;
%             $worklist$.add($block$)\;
%         }
%     }
% }

% \BlankLine
% \Fn{\AnalyzeBlock{$block$}}{
%     $du\_chain \leftarrow$ empty DUChain\;
%     \ForEach{statement $stmt$ in $block$}{
%         \If{$stmt$.is\_assignment()}{
%             $du\_chain$.add\_definition($stmt$.get\_assigned\_variable(), $stmt$)\;
%         }
%         \If{$stmt$.is\_expression()}{
%             $du\_chain$.add\_use($stmt$.get\_used\_variables(), $stmt$)\;
%         }
%     }
%     \Return $du\_chain$\;
% }

% \BlankLine
% \Fn{\IsDeadCode{$stmt$, $du\_chain$}}{
%     \If{$stmt$.is\_assignment()}{
%         $var \leftarrow stmt$.get\_assigned\_variable()\;
%         \Return \textbf{not} $du\_chain$.is\_used($var$)\;
%     }
%     \Return \textbf{false}\;
% }

% \BlankLine
% \Fn{\RemoveStmt{$block$, $stmt$}}{
%     $block$.remove($stmt$)\;
% }
% \end{algorithm}

\begin{algorithm}
\caption{Unused Code Elimination}
\label{alg:unused_code}
\KwIn{program}
\KwOut{program with unused code eliminated}
\SetKwProg{Fn}{Function}{:}{end}
\SetKwFunction{InitWorklist}{init\_worklist}
\SetKwFunction{RemoveStmt}{remove\_statement}
\SetKwFunction{buildDUChain}{buildDefUseChains}
\Begin{
    DUChain$\leftarrow$\buildDUChain{$program$}\;
    \InitWorklist{$worklist$, $program$}\;
        
    \While{worklist is not empty}{
        $stmt$ $\leftarrow$ worklist.pop()\;
        \tcp{Get variables defined in stmt}
        \ForEach{var $\in$ Def(stmt)}{
            \ForEach{useStmt $\in$ DUChain[var].uses}{
                \If{not useStmt.useful}{
                    useStmt.useful $\leftarrow$ true\;
                    worklist.append(useStmt)\;
                }
            }
        }
    }
    \tcp{Remove unused statements}
    \ForEach{stmt $\in$ program}{
        \If{not stmt.useful}{
            \RemoveStmt{program, stmt}\;
        }
    }

    \Return{program}\;
}

\BlankLine
\Fn{\buildDUChain{$program$}}{
    DUChain $\leftarrow$ InitializeEmptyDefUseChain()\;
    
    \ForEach{statement $\in$ program}{
        \ForEach{variable $\in$ Def(statement)}{
            DUChain[variable].defs.add(statement)\;
        }
        
        \ForEach{variable $\in$ Use(statement)}{
            DUChain[variable].uses.add(statement)\;
        }
    }
    
    \Return{DUChain}\;
}

\end{algorithm}


==> figures/case_study_locale_charset.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
            \begin{minted}[]{c}
char const *locale_charset(void) {
    ...
    codeset = (char const *)nl_langinfo(14);
    if ((unsigned long)codeset 
         == (unsigned long)((void *)0)) {
        codeset = "";
    }
    aliases = get_charset_aliases();
    while (1) {
        ... // Handing aliases
    }
    ... 
    return (codeset);
}
\end{minted}
        \caption{The debloated function produced by CovA}
        \label{subfig:locale_cova}
    \end{subfigure}

     \begin{subfigure}[b]{0.45\textwidth}
            \begin{minted}[breaklines]{c}
char const *locale_charset(void) {
    char const *codeset = nl_langinfo(14);
    return (codeset == NULL || codeset[0] == '\0') ? "ASCII" : codeset;
}
\end{minted}
        \caption{The debloated function produced by \toolname}
        \label{subfig:locale_tool}
    \end{subfigure}
    \caption{The debloated {\tt locale\_charset} generated by CovA and \toolname}
    \label{fig:case_study_locale}
\end{figure}


==> figures/motivation.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
            \begin{minted}[highlightcolor=lightgreen,highlightlines={3-7}]{c}
char const *locale_charset(void) {
    ...
    codeset = (char const *)nl_langinfo(14);
    if ((unsigned long)codeset 
         == (unsigned long)((void *)0)) {
        codeset = "";
    }
\end{minted}
\begin{minted}[highlightcolor=lightred,highlightlines={1-4}]{c}
    aliases = get_charset_aliases();
    while (1) {
        ... // Handing aliases
    }
    ... 
    return (codeset);
}
\end{minted}
        \caption{The code snippet of {\tt locale\_charset}}
        \label{subfig:locale}
    \end{subfigure}

     \begin{subfigure}[b]{0.45\textwidth}
            \begin{minted}[]{c}
static char const *gettext_quote(...) {
    ...
    loc_code = locale_charset();
    tmp_1 = c_strcasecmp(loc_code,"UTF-8");
    tmp_3 = c_strcasecmp(loc_code,"GB18030");
    ...
}
\end{minted}
        \caption{The callee of {\tt locale\_charset}}
        \label{subfig:locale_callee}
    \end{subfigure}
    

    \caption{The {\tt locale\_charset} and its callee in {\tt date} program}
    \label{fig:enter-label}
\end{figure}


==> figures/motivation_less_cases.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
            \begin{minted}[highlightcolor=lightgreen,highlightlines={3-7}]{c}
char const *locale_charset(void) {
    ...
    codeset = (char const *)nl_langinfo(14);
    if ((unsigned long)codeset 
         == (unsigned long)((void *)0)) {
        codeset = "";
    }
\end{minted}
\begin{minted}[highlightcolor=lightred,highlightlines={1-4}]{c}
    aliases = get_charset_aliases();
    while (1) {
        ... // Handing aliases
    }
    ... 
    return (codeset);
}
\end{minted}
        \caption{The code snippet of {\tt locale\_charset}}
        \label{subfig:locale}
    \end{subfigure}

     \begin{subfigure}[b]{0.45\textwidth}
            \begin{minted}[]{c}
static char const *gettext_quote(...) {
    ...
    loc_code = locale_charset();
    tmp_1 = c_strcasecmp(loc_code,"UTF-8");
    tmp_3 = c_strcasecmp(loc_code,"GB18030");
    ...
}
\end{minted}
        \caption{The callee of {\tt locale\_charset}}
        \label{subfig:subfig_callee}
    \end{subfigure}
    

    \caption{The {\tt locale\_charset} and its callee in {\tt date} program}
    \label{fig:enter-label}
\end{figure}


==> figures/motivation_more_cases.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \begin{minted}[breaklines,fontsize=\small]{c}
int yyparse(parser_control *pc) {
  ...
  case_23:
    set_hhmmss(pc, (yyvsp + -3)->textintval.value,
               (yyvsp + -1)->textintval.value, (time_t)0, 0L);
    pc->meridian = 2;
    goto switch_break;
  ...
}
        \end{minted}
        \caption{The code snippet of {\tt yyparse}}
        \label{subfig:yyparse}
    \end{subfigure}

     \begin{subfigure}[b]{0.45\textwidth}
            \begin{minted}[]{c}

// Observed input
date -d "2010-02-07 12:10:53"
\end{minted}
        \caption{The observed input}
        \label{subfig:input_cases}
    \end{subfigure}

    \caption{The {\tt yyparse} and corresponding inputs in {\tt date} program}
    \label{fig:enter-label}
\end{figure}

% // Unovserved input
% date -d "16:30 next Monday"

==> listings/code_case_1.tex <==
def iseq(start=0, stop=None, inc=1):
    if stop is None:
        stop = start
        start = 0
        inc = 1
    return arange(start, stop+inc, inc)

==> listings/code_case_2.tex <==
def poke(self, context):
    message = self.pubsub.get_message()
    if message and message['type'] == 'message':
        context['ti'].xcom_push(key='message', value=message)
        self.pubsub.unsubscribe(self.channels)
        return True
    return False

==> prompts/program_understanding_prompt.tex <==
\prompt{Prompt: Program Understanding}{1}{
You are tasked with analyzing the main function of a program using your knowledge to extract its functionalities, supported options, and use cases.\\

\textbf{\# Task}\\
For the provided main function, perform the following steps:\\
\hspace{10pt}-Identify Core Features: Based on the structure of the main function, its arguments, and your knowledge, infer the primary functionalities of the program.

\hspace{10pt}-Extract Supported Command-Line Options: Identify and describe any command-line options or arguments used in the main function’s code. Include explanations for each option’s purpose.

\hspace{10pt}-Explain Core Use Cases: Using the main function’s logic and arguments, summarize the typical use cases or tasks the program likely supports.
\\

\textbf{\# Input}\\
The following code is the main function of \{PROGRAM NAME\}:\\
\{MAIN FUNCTION\}
\\

\textbf{\# Output}\\
For each feature identified:\\
\hspace{10pt}-Provide a description of the feature based on the main function's logic.\\
\hspace{10pt}-List the command-line options and explain them. \\
\hspace{10pt}-Summarize the core use cases supported by the program, including typical input/output scenarios.

}

